Beyond Diagonal RIS-Aided Networks: Performance Analysis and Sectorization Tradeoff

Reconfigurable intelligent surfaces (RISs) have emerged as a spectrum- and energy-efficient technology to enhance the coverage of wireless communications within the upcoming 6G networks. Recently, novel extensions of this technology, referred to as multi-sector beyond diagonal RIS (BD-RIS), have been proposed, where the configurable elements are divided into $L$ sectors $(L \geq 2)$ and arranged as a polygon prism, with each sector covering $1/L$ space. This paper presents a performance analysis of a multi-user communication system assisted by a multi-sector BD-RIS operating in time-switching (TS) mode. Specifically, we derive closed-form expressions for the moment-generating function (MGF), probability density function (PDF), and cumulative density function (CDF) of the signal-to-noise ratio (SNR) per user. Furthermore, closed-form expressions for the outage probability, achievable spectral and energy efficiency, symbol error probability, and diversity order for the proposed system model are derived. Moreover, a comparison is performed with the simultaneously transmitting and reflecting (STAR)-RISs, a special case of multi-sector BD-RIS with two sectors. Our analysis shows that for a fixed number of elements, increasing the sectors improves outage performance at the expense of reduced diversity order compared to STAR-RIS. This trade-off is influenced by the Rician factors of the cascaded channel and the number of configurable elements per sector. However, this superiority in slope is observed at outage probability values below $10^{-5}$, which remains below practical operating ranges of communication systems. Additionally, simulations are provided to validate the accuracy of our theoretical analyses showing a notable $182\%$ increase in spectral efficiency and a $238\%$ increase in energy efficiency when transitioning from a 2-sector to a 6-sector configuration.

==> Energy_eff/EE3.tex <==
\begin{figure}[t]
\centering
\scalebox{\sca}{\begin{tikzpicture}
\begin{axis}[
        xmin=0, xmax=10,        ymin=0, ymax=30,
    xlabel={\xyfont Achievable SE (bit/s/Hz)},       ylabel={\xyfont Achievable EE (Mb/J)},
    xlabel style={black, font=\fontfamily{cmr}\footnotesize , yshift=0mm},
    ylabel style={black, font=\fontfamily{cmr}\footnotesize, yshift=-1.5mm},
    y tick label style={black, font=\fontfamily{ppl}\tickfont , xshift=0.75mm},
    x tick label style={black, font=\fontfamily{ppl}\tickfont , yshift=0mm},
 grid=both, \majorgrid,  \minorgrid,
legend style={at={(axis cs:10,30)},anchor=north east},
 legend style={font=%\fontfamily{cmr}
\fontsize{7pt}{2pt}\selectfont,inner sep=0pt,outer sep=0pt},legend image post style={scale=0.8},  %%% <--- here
               width=8.4cm,             height=7cm,  
legend cell align={left}, legend entries={
Analysis $L=6$,
Analysis $L=5$,
Analysis $L=4$,
Analysis $L=3$,
Analysis $L=2$,
simulation},
 %title style={yshift=1cm}, title= {Figure 2},
 ]
]


\color{black}
 % For legendry colors
 \usetikzlibrary{shapes}

\addplot[line width=1pt,color=red, mark=o, mark size=2.5pt, mark options=solid,solid] coordinates{ (-50, 1)};

% TEAL
\addplot[line width=1pt,color=teal, mark=pentagon, mark size=3.0pt,mark options=solid] coordinates{ (-50, 1)};

% CYAN
\addplot[line width=1pt,color=cyan, mark=triangle, mark size=3.0pt]
coordinates{(-50, 1)};

% MAGENTA
\addplot[line width=1pt,color=magenta, mark=diamond, mark size=3.5pt, mark options=solid,solid] coordinates{ (-50, 1)};

% BLUE 
\addplot[line width=1pt,color=blue, mark=square, mark size=2.75pt, mark options=solid,solid] coordinates{ (-50, 1)};

% STAR
\addplot[line width=1pt,color=black,mark=*, mark size=1.5pt, mark options=solid,solid, only marks] coordinates{ (-50, 1)};


\iffalse
no_U=10**(      (no_dBm-30)/10        )
K=6
sectors =[3, 4, 5, 6]
dh, dg = 100, 30
Kh, Kg= 10, 10
elements=360/L
\fi
%10 users
\color{black}
 % For legendry colors
 \usetikzlibrary{shapes}

\addplot[line width=1pt,color=red, mark=o, mark size=2.5pt, mark options=solid,solid] coordinates{ (-50, 1)};

% TEAL
\addplot[line width=1pt,color=teal, mark=pentagon, mark size=3.0pt,mark options=solid] coordinates{ (-50, 1)};

% CYAN
\addplot[line width=1pt,color=cyan, mark=triangle, mark size=3.0pt]
coordinates{(-50, 1)};

% MAGENTA
\addplot[line width=1pt,color=magenta, mark=diamond, mark size=3.5pt, mark options=solid,solid] coordinates{ (-50, 1)};

% BLUE 
\addplot[line width=1pt,color=blue, mark=square, mark size=2.75pt, mark options=solid,solid] coordinates{ (-50, 1)};

% STAR
\addplot[line width=1pt,color=black,mark=*, mark size=1.5pt, mark options=solid,solid, only marks] coordinates{ (-50, 1)};







\iffalse %%%%%
K=50 %%%%%
\fi%%%%%%%%%%
\iffalse
L=2
\fi
\addplot[line width=1.1pt,color=blue, mark=square, mark options=solid,solid] 
table[x=x, y=y1]{./Energy_eff/EE3.txt};
\addplot[line width=0.5pt,color=black,mark=*, mark size=1pt, only marks] 
table[x=x, y=y_sim1]{./Energy_eff/EE3.txt};


\iffalse
L=3
\fi
% cascaded
\addplot[line width=1pt,color=magenta, mark=diamond, mark size=3.25pt, mark options=solid,solid]
table[x=x, y=y2]{./Energy_eff/EE3.txt};
\addplot[line width=0.5pt,color=black,mark=*, mark size=1pt, only marks] 
table[x=x, y=y_sim2]{./Energy_eff/EE3.txt};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
L=4
\fi
% cascaded
\addplot[line width=1.1pt,color=cyan, mark=triangle, mark size=3.5, mark options=solid,solid] 
table[x=x, y=y3]{./Energy_eff/EE3.txt};

\addplot[line width=0.5pt,color=black,mark=*, mark size=1pt, only marks] 
table[x=x, y=y_sim3]{./Energy_eff/EE3.txt};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
L=5
\fi
% cascaded
\addplot[line width=1.1pt,color=teal, mark=pentagon, mark size=3.25,mark options=solid]
table[x=x, y=y4]{./Energy_eff/EE3.txt};

\addplot[line width=0.5pt,color=black,mark=*, mark size=1pt, only marks] 
table[x=x, y=y_sim4]{./Energy_eff/EE3.txt};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
L=6
\fi
% cascaded
\addplot[line width=1.1pt,color=red, mark=o, mark size=2.5, mark options=solid,solid] 
table[x=x, y=y5]{./Energy_eff/EE3.txt};
\addplot[line width=0.5pt,color=black,mark=*, mark size=1pt, only marks] 
table[x=x, y=y_sim5]{./Energy_eff/EE3.txt};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\end{axis}
\end{tikzpicture}}
\vspace{-1.0mm}
\renewcommand{\figurename}{\footnotesize Fig.}
\captionwidth
\caption{\footnotesize Energy efficiency versus spectral efficiency for fixed total number of elements for the whole multi-sector $LM=360$ with different number of sectors, $P_e=0.5$ mW, and $\kappa_h=\kappa_g=10$.}
\label{se_eff}
\vspace{-1mm}
\end{figure}


==> Outage/Asymbtotic.tex <==
\begin{figure}[t]
\centering
\scalebox{\sca}{\begin{tikzpicture}
\begin{semilogyaxis}[
        xmin=0, xmax=50,        ymin=1e-200, ymax=1e0,
    xlabel={\xyfont Transmit Power (dBm)},       ylabel={\xyfont Outage Probability},
    xlabel style={black, font=\fontfamily{cmr}\footnotesize , yshift=0mm},
    ylabel style={black, font=\fontfamily{cmr}\footnotesize, yshift=-1.5mm},
    y tick label style={black, font=\fontfamily{ppl}\tickfont , xshift=0.75mm},
    x tick label style={black, font=\fontfamily{ppl}\tickfont , yshift=0mm},
 grid=both, \majorgrid,  \minorgrid,
legend style={at={(axis cs:0,1e-200)},anchor=south west},
 legend style={font=%\fontfamily{cmr}
\fontsize{7pt}{2pt}\selectfont,inner sep=0pt,outer sep=0pt},legend image post style={scale=0.8},  %%% <--- here
               width=8.4cm,             height=7cm,  
legend cell align={left}, legend entries={ 
Asymptotic,
Analysis,
Simulation}]


\color{black}
 % For legendry colors
 \addplot[line width=1.1pt,color=blue,dashed]coordinates{(-50, 1)};
\addplot[line width=1pt,color=black] coordinates{ (-50, 1)};
\addplot[line width=1pt,color=black,mark=asterisk, only marks, mark size=2pt, only marks]coordinates{ (-50, 1)};


\addplot[line width=1.1pt,color=red,dashed]coordinates{(-50, 1)};
\addplot[line width=1pt,color=orange] coordinates{ (-50, 1)};
\addplot[line width=1pt,color=orange,mark=asterisk, only marks, mark size=2pt, only marks]coordinates{ (-50, 1)};

\iffalse
no_U=10**(      (no_dBm-30)/10        )
K=6
sectors =[3, 4, 5, 6]
dh, dg = 100, 30
Kh, Kg= 10, 10
elements=360/L
\fi
%10 users
\color{black}
 % For legendry colors
 \usetikzlibrary{shapes}

\addplot[line width=1pt,color=blue, mark=o, mark size=2.5pt, mark options=solid,solid] coordinates{ (-50, 1)};

% TEAL
\addplot[line width=1pt,color=teal, mark=pentagon, mark size=3.0pt,mark options=solid] coordinates{ (-50, 1)};

% CYAN
\addplot[line width=1pt,color=cyan, mark=triangle, mark size=3.0pt]
coordinates{(-50, 1)};

% MAGENTA
\addplot[line width=1pt,color=magenta, mark=diamond, mark size=3.5pt, mark options=solid,solid] coordinates{ (-50, 1)};

% BLUE 
\addplot[line width=1pt,color=blue, mark=square, mark size=2.75pt, mark options=solid,solid] coordinates{ (-50, 1)};

% STAR
\addplot[line width=1pt,color=black,mark=*, mark size=1.5pt, mark options=solid,solid, only marks] coordinates{ (-50, 1)};







\iffalse %%%%%
K=50 %%%%%
\fi%%%%%%%%%%
\iffalse
L=2
\fi
\addplot[line width=1.1pt,color=black]
table[x=x, y=y1]{./Outage/Asymbtotic.txt};
 \addplot[line width=1.1pt,color=blue, mark size=2.5,mark options=solid,dashed] 
table[x=x, y=y_sim1]{./Outage/Asymbtotic.txt};


\iffalse
L=3
\fi
% cascaded
\addplot[line width=1.1pt,color=black]
table[x=x, y=y2]{./Outage/Asymbtotic.txt};
 \addplot[line width=1.1pt,color=blue, mark size=2.5,mark options=solid,dashed] 
table[x=x, y=y_sim2]{./Outage/Asymbtotic.txt};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
L=4
\fi
% cascaded
\addplot[line width=1.1pt,color=black]
table[x=x, y=y3]{./Outage/Asymbtotic.txt};

 \addplot[line width=1.1pt,color=blue, mark size=2.5,mark options=solid,dashed] 
table[x=x, y=y_sim3]{./Outage/Asymbtotic.txt};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
L=5
\fi
% cascaded
\addplot[line width=1.1pt,color=black]
table[x=x, y=y4]{./Outage/Asymbtotic.txt};

 \addplot[line width=1.1pt,color=blue, mark size=2.5,mark options=solid,dashed] 
table[x=x, y=y_sim4]{./Outage/Asymbtotic.txt};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
L=6
\fi
% cascaded
\addplot[line width=1.1pt,color=black]
table[x=x, y=y5]{./Outage/Asymbtotic.txt};
 \addplot[line width=1.1pt,color=blue, mark size=2.5,mark options=solid,dashed] 
table[x=x, y=y_sim5]{./Outage/Asymbtotic.txt};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\node[align=left,fill=white] at (axis cs:34.01,1e-75){\fontsize{8.5pt}{2pt}\selectfont $LM_l\mkern-3mu=\mkern-3mu
60,
\mkern-5mu
~120,
\mkern-5mu
~180,
\mkern-5mu
~240,
\mkern-5mu
~360$};
\draw[->, >=stealth,line width=0.8pt](axis cs:36.01,1e-82) to (axis cs:10.01,1e-150);

\end{semilogyaxis}
\end{tikzpicture}}
\vspace{-3.0mm}
\renewcommand{\figurename}{\footnotesize Fig.}
\captionwidth
\caption{\footnotesize Achievable rate per user vs $p$ in dBm for different number of users per time frame with $M=32$ and $\kappa_h=\kappa_g=10$.}
\label{asymLM}
\vspace{-1mm}
\end{figure}

==> Outage/Ric_Asym.tex <==
\begin{figure}[t]
\centering
\scalebox{\sca}{\begin{tikzpicture}
\begin{semilogyaxis}[
        xmin=0, xmax=50,        ymin=1e-200, ymax=1e0,
    xlabel={\xyfont Transmit Power (dBm)},       ylabel={\xyfont Outage Probability},
    xlabel style={black, font=\fontfamily{cmr}\footnotesize , yshift=0mm},
    ylabel style={black, font=\fontfamily{cmr}\footnotesize, yshift=-1.5mm},
    y tick label style={black, font=\fontfamily{ppl}\tickfont , xshift=0.75mm},
    x tick label style={black, font=\fontfamily{ppl}\tickfont , yshift=0mm},
 grid=both, \majorgrid,  \minorgrid,
legend style={at={(axis cs:50,1e-200)},anchor=south east},
 legend style={font=%\fontfamily{cmr}
\fontsize{7pt}{2pt}\selectfont,inner sep=0pt,outer sep=0pt},legend image post style={scale=0.8},  %%% <--- here
               width=8.4cm,             height=7cm,  
legend cell align={left}, legend entries={ 
Asymptotic,
Analysis,
Simulation}]


\color{black}
 % For legendry colors
 \addplot[line width=1.1pt,color=red,dashed]coordinates{(-50, 1)};
\addplot[line width=1pt,color=black] coordinates{ (-50, 1)};
\addplot[line width=1pt,color=black,mark=asterisk, only marks, mark size=2pt, only marks]coordinates{ (-50, 1)};


\color{black}
\usetikzlibrary{shapes}



\node[align=left,fill=white] at (axis cs:42.5,8.0e-60){\fontsize{7.5pt}{2pt}\selectfont ~~~$\kappa\mkern-2mu=\mkern-2mu0$\\ \fontsize{7.5pt}{2pt}\selectfont~~~$\eta\mkern-2mu=\mkern-2mu
3$};



\node[align=left,fill=white] at (axis cs:30.5,1.0e-100){\fontsize{7.5pt}{2pt}\selectfont ~~$\kappa\mkern-2mu=\mkern-2mu5$\\ \fontsize{7.5pt}{2pt}\selectfont~~~$\eta\mkern-2mu=\mkern-2mu2.5$};



\node[align=left,fill=white] at (axis cs:12.5,1.0e-140){\fontsize{7.5pt}{2pt}\selectfont ~~$\kappa\mkern-2mu=\mkern-2mu10$\\ \fontsize{7.5pt}{2pt}\selectfont~~~$\eta\mkern-2mu=\mkern-2mu2$};







\iffalse
no_U=10**(      (no_dBm-30)/10        )
K=6
sectors =[3, 4, 5, 6]
dh, dg = 100, 30
Kh, Kg= 10, 10
elements=360/L
\fi


\addplot[line width=1.1pt,color=red,dashed] 
table[x=x, y=y_asym1]{./Outage/Ric_Asym.txt};


\addplot[line width=1.1pt,color=black] 
table[x=x, y=y1]{./Outage/Ric_Asym.txt};

\addplot[line width=1.1pt,color=black, mark=asterisk, only marks, mark size=2.5,mark options=solid] 
table[x=x, y=y_sim1]{./Outage/Ric_Asym.txt};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot[line width=1.1pt,color=red,dashed] 
table[x=x, y=y_asym2]{./Outage/Ric_Asym.txt};


\addplot[line width=1.1pt,color=black] 
table[x=x, y=y2]{./Outage/Ric_Asym.txt};

\addplot[line width=1.1pt,color=black, mark=asterisk, only marks, mark size=2.5,mark options=solid] 
table[x=x, y=y_sim2]{./Outage/Ric_Asym.txt};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addplot[line width=1.1pt,color=red,dashed] 
table[x=x, y=y_asym3]{./Outage/Ric_Asym.txt};


\addplot[line width=1.1pt,color=black] 
table[x=x, y=y3]{./Outage/Ric_Asym.txt};

\addplot[line width=1.1pt,color=black, mark=asterisk, only marks, mark size=2.5,mark options=solid] 
table[x=x, y=y_sim3]{./Outage/Ric_Asym.txt};




\end{semilogyaxis}
\end{tikzpicture}}
\vspace{-2.0mm}
\renewcommand{\figurename}{\footnotesize Fig.}
\captionwidth
\caption{\footnotesize Asymptotic outage analysis and simulation for muli-sector BD-RIS with different numbers of sectors, and different Rician factors $\kappa_g=\kappa_h=\kappa$ for $R_l = 0.25$, and for $L=6$.}
\label{asym_RI}
\vspace{-1mm}
\end{figure}

==> System_model/operation_modes.tex <==
%\begin{figure}
%\centering
\scalebox{1}{\begin{overpic}[width=\linewidth]{System model/modes.pdf}


\put(7,41.9){\fontsize{10.0pt}{2pt}\selectfont $\beta_{l,m}=1$} 


\put(7,38.0){\fontsize{10.0pt}{2pt}\selectfont $\beta_{l,m}=0$} 

\put(7,33.8){\fontsize{10.0pt}{2pt}\selectfont $0>\beta_{l,m}>1$} 


\put(8,2.8){\footnotesize (a) Energy splitting} 
\put(45,2.8){\footnotesize (b) Sector switching} 
\put(80,2.8){\footnotesize (c) Group splitting} 


\end{overpic}}
          \vspace{-0.6mm}
\renewcommand{\figurename}{\footnotesize Fig}
      \caption{\footnotesize Different operational modes for the multi-sector BD-RIS with $L=3$}
       \vspace{-2.6mm}
          \label{modes_op}
%\end{figure}


